DeepBlur: A Simple and Effective Method for Natural Image Obfuscation

There is a growing privacy concern due to the popularity of social media and surveillance systems, along with advances in face recognition software. However, established image obfuscation techniques are either vulnerable to re-identification attacks by human or deep learning models, insufficient in preserving image fidelity, or too computationally intensive to be practical. To tackle these issues, we present DeepBlur, a simple yet effective method for image obfuscation by blurring in the latent space of an unconditionally pre-trained generative model that is able to synthesize photo-realistic facial images. We compare it with existing methods by efficiency and image quality, and evaluate against both state-of-the-art deep learning models and industrial products (e.g., Face++, Microsoft face service). Experiments show that our method produces high quality outputs and is the strongest defense for most test cases.

==> figures_comparison.tex <==
\begin{figure*}[!ht]
\begin{center}
\setlength{\tabcolsep}{.15em}
\begin{tabular}{ccccccc}
    $Original$ & $Blurred$ & $Pixelated$ & $Masking$ & $Fawkes$~\cite{shan2020fawkes} & $Ours^\dagger$ & $Ours^\ddagger$ \\
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_chan.png}
    & 
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_chan_blur.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_chan_pixelate.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_chan_mask.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_chan_cloaked.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_chan_0.50.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_chan_1.00.png}
    \\
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_portman.png}
    & 
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_portman_blur.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_portman_pixelate.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_portman_mask.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_portman_cloaked.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_portman_0.50.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_portman_1.00.png}
    \\
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_washington.png}
    & 
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_washington_blur.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_washington_pixelate.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_washington_mask.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_washington_cloaked.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_washington_0.50.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_washington_1.00.png}
    \\
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_berry.png}
    & 
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_berry_blur.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_berry_pixelate.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_berry_mask.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_berry_cloaked.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_berry_0.50.png}
    & \hspace{\sizeHorizontalSpace}
    \includegraphics[width=\sizeImage\textwidth]{images_comparison_berry_1.00.png}
\end{tabular}
\end{center}
\caption{Comparison of different obfuscation methods.}
\label{fig:comparison}
\end{figure*}


==> figures_metrics.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.31\textwidth]{images_plot_ssim_fid_vs_sigma.png}
\caption{
    SSIM and FID changing monotonically with $\sigma$. 
}
\label{fig:metrics}
\end{figure}



==> sections_acknowledgment.tex <==
\section{Acknowledgment}\label{sec:acknowledgment}
\section{Final copy}

You must include your signed IEEE copyright release form when you submit
your finished paper. We MUST have this form before your paper can be
published in the proceedings.

Please direct any questions to the production editor in charge of these
proceedings at the IEEE Computer Society Press: 
\url{https://www.computer.org/about/contact}.



==> tables_accuracies.tex <==
\begin{table*}[]
\begin{center}
\begin{tabular}{llllllll}
\hline
\multirow{2}{*}{Model}     & \multirow{2}{*}{setting} & \multicolumn{2}{l}{VGG19} & \multicolumn{2}{l}{ResNet18} & \multirow{2}{*}{Face++} & \multirow{2}{*}{MS Azure} \\
                           &                          & acc@1       & acc@5       & acc@1         & acc@5        &                         &                           \\ \hline
clear                      & -                        &             &             &               &              & 97.3                        & 93.5                          \\ \hline
pixelate\_32               & -                        &             &             &               &              & 3.4                        & 25.5                          \\ \hline
blur\_50                   & -                        &             &             &               &              & 92.2                        & 59.2                          \\ \hline
p3\_20                     & -                        &             &             &               &              &                         &                           \\ \hline
mask                       & -                        &             &             &               &              & 51.4                        & 28.9                          \\ \hline
\multirow{3}{*}{Fawkes}    & low                      &             &             &               &              & 95.1                        & 76.5                          \\
                           & mid                      &             &             &               &              &                         &                           \\
                           & high                     &             &             &               &              &                         &                           \\ \hline
\multirow{3}{*}{Deep-Blur} & 0.5                      &             &             &               &              & 62.2                        & 33.0                          \\
                           & 1.0                      &             &             &               &              & 5.8                        & 0.0                          \\
                           & 2.0                      &             &             &               &              & 1.4                        & 0.0                          \\ \hline
\end{tabular}
\end{center}
\caption{clean-to-obfuscate accuracy comparision (currently it's a placeholder)}
\label{tab:accuracies}
\end{table*}


==> tables_accuracies2.tex <==
\begin{table*}[]
\begin{tabular}{llllllll}
\hline
\multirow{2}{*}{Model}     & \multirow{2}{*}{setting} & \multicolumn{2}{l}{VGG19} & \multicolumn{2}{l}{ResNet18} & \multirow{2}{*}{Face++} & \multirow{2}{*}{MS Azure} \\
                           &                          & acc@1       & acc@5       & acc@1         & acc@5        &                         &                           \\ \hline
clear                      & -                        &             &             &               &              & 97.3                        & 93.5                          \\ \hline
pixelate\_32               & -                        &             &             &               &              & 0.0*                        & 39.1                          \\ \hline
blur\_50                   & -                        &             &             &               &              & 94.2                        & 68.4                          \\ \hline
p3\_20                     & -                        &             &             &               &              &                         &                           \\ \hline
mask                       & -                        &             &             &               &              & 64.6                        & 20.0                          \\ \hline
\multirow{3}{*}{Fawkes}    & low                      &             &             &               &              & 90.8                        & 85.7                          \\
                           & mid                      &             &             &               &              &                         &                           \\
                           & high                     &             &             &               &              &                         &                           \\ \hline
\multirow{3}{*}{Deep-Blur} & 0.5                      &             &             &               &              & 90.8                        & 50.0                          \\
                           & 1.0                      &             &             &               &              & 18.0                        & 0.0                          \\
                           & 2.0                      &             &             &               &              & 3.7                        & 0.0                          \\ \hline
\end{tabular}
\label{tab:accuracies2}
\caption{obfuscate-to-clean accuracy comparision (currently it's a placeholder). *Face$^{++}$ couldn't detect face from pixelated images, thus did not learn anything.}
\end{table*}


==> tables_accuracies3.tex <==
\begin{table*}[]
\begin{tabular}{llllllll}
\hline
\multirow{2}{*}{Model}     & \multirow{2}{*}{setting} & \multicolumn{2}{l}{VGG19} & \multicolumn{2}{l}{ResNet18} & \multirow{2}{*}{Face++} & \multirow{2}{*}{MS Azure} \\
                           &                          & acc@1       & acc@5       & acc@1         & acc@5        &                         &                           \\ \hline
clear                      & -                        &             &             &               &              & 97.3                        & 93.5                          \\ \hline
pixelate\_32               & -                        &             &             &               &              & 0.0*                        & 65.3                         \\ \hline
blur\_50                   & -                        &             &             &               &              & 91.2                        & 87.0                          \\ \hline
p3\_20                     & -                        &             &             &               &              &                         &                           \\ \hline
mask                       & -                        &             &             &               &              & 44.9                        & 5.1                          \\ \hline
\multirow{3}{*}{Fawkes}    & low                      &             &             &               &              & 88.9                        & 74.3                          \\
                           & mid                      &             &             &               &              &                         &                           \\
                           & high                     &             &             &               &              &                         &                           \\ \hline
\multirow{3}{*}{Deep-Blur} & 0.5                      &             &             &               &              & 49.3                        & 45.6                         \\
                           & 1.0                      &             &             &               &              & 6.8                        & 12.6                          \\
                           & 2.0                      &             &             &               &              & 2.0                        & 4.4                          \\ \hline
\end{tabular}
\label{tab:accuracies3}
\caption{obfuscate-to-obfuscate accuracy comparision (currently it's a placeholder). *Face$^{++}$ couldn't detect face from pixelated images, thus did not learn anything.}
\end{table*}


==> tables_accuracies_merged2.tex <==
\begin{table*}[]
\begin{center}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{@{}ccccccccccccc@{}}
\toprule
           & \multicolumn{4}{c}{Threat Model $T_1$}         & \multicolumn{4}{c}{Threat Model $T_2$}          & \multicolumn{4}{c}{Threat Model $T_3$}         \\ \cmidrule(l){2-13}
           & VGG19 & ResNet18 & Face++       & Azure        & VGG19 & ResNet18 & Face++        & Azure        & VGG19 & ResNet18 & Face++       & Azure        \\ \midrule
Original   &       &          & 97.3         & 93.5         &       &          & 97.3          & 93.5         &       &          & 97.3         & 93.5         \\
Pixelation &       &          & 45.8 & 25.5         &       &          & \textbf{11.6}             & 39.1         &       &          & 29.2            & 65.3         \\
Blurring   &       &          & 92.2         & 59.2         &       &          & 94.2          & 68.4         &       &          & 91.2         & 87.1         \\
Masking    &       &          & 61.4         & 28.9         &       &          & 64.6          & 20.1        &       &          & 53.7         & \textbf{5.1} \\
AdvNoise   &       &          & 95.1         & 74.0         &       &          & 90.8          & 87.8         &       &          & 91.0         & 76.0         \\
DeepBlur$^\dagger$ &       &          & 68.3         & 33.0         &       &          & 90.8          & 50.0         &       &          & 54.1         & 46.0         \\
DeepBlur$^\ddagger$&       &          & \textbf{6.0}          & \textbf{0.0} &       &          & 18.0 & \textbf{0.0} &       &          & \textbf{7.0} & 12.6         \\ \bottomrule
\end{tabular}%
}
\end{center}
\caption{
    Comparison of obfuscation methods.
    We evaluate the performance of the obfuscation methods by top-1 accuracies 
    from four face recognition systems (i.e., VGG19, ResNet18, Face++, Microsoft Azure Face API) under different threat model settings.
    For DeepBlur, we evaluate the cases of $\sigma = 0.5$ and $\sigma = 1.0$ (the same settings as in \cref{fig:teaser,fig:deepblur_demo})
    and show that it is the strongest defense at most times.
    Note that Face++ cannot be trained on pixelated images as it cannot detect faces from them.
}
\label{tab:accuracies_merged}
\end{table*}

